MarQSim: Reconciling Determinism and Randomness in Compiler Optimization for Quantum Simulation

Quantum simulation, fundamental in quantum algorithm design, extends far beyond its foundational roots, powering diverse quantum computing applications. However, optimizing the compilation of quantum Hamiltonian simulation poses significant challenges. Existing approaches fall short in reconciling deterministic and randomized compilation, lack appropriate intermediate representations, and struggle to guarantee correctness. Addressing these challenges, we present MarQSim, a novel compilation framework. MarQSim leverages a Markov chain-based approach, encapsulated in the Hamiltonian Term Transition Graph, adeptly reconciling deterministic and randomized compilation benefits. We rigorously prove its algorithmic efficiency and correctness criteria. Furthermore, we formulate a Min-Cost Flow model that can tune transition matrices to enforce correctness while accommodating various optimization objectives. Experimental results demonstrate MarQSim's superiority in generating more efficient quantum circuits for simulating various quantum Hamiltonians while maintaining precision.

==> tex/8-Conclusion.tex <==
\section{Conclusion}


In this paper, we present a pragmatic quantum compiler - Markov simulation, for the quantum simulation operator $e^{iHt}$. This development is an extension of Earl Campbell's seminal work \cite{campbell2019random}. Unlike Campbell's approach, Markov simulation incorporates local quantum circuit optimization, striking a balance between algorithmic and physical error. The underpinning concept of our co-optimization strategy is inspired by the Markov process and the minimum-cost flow problem.

Subsequently, we subject a variety of quantum simulation tasks to evaluation on classical computers. The results obtained distinctly indicate our method's superiority over the original work, particularly in scenarios involving Hamiltonians with relatively long Pauli strings. These promising outcomes lend credence to our conjecture that our approach could yield even better performance in practical situations, where the length of Pauli strings invariably exceeds the parameters of our evaluation.
